The role of central places in exposure segregation

Here we show that "exposure segregation" - the degree to which individuals of one group are exposed to individuals of another in day-to-day mobility - is dependent on the structure of cities, and the importance of downtowns in particular. Recent work uses aggregated data to claim that the location of amenities can inhibit or facilitate interactions between groups: if a city is residentially segregated, as many American cities are, then amenities between segregated communities should encourage them to mix. We show that the relationship between "bridging" amenities and socio-economic mixing breaks down when we examine the amenities themselves, rather than the urban aggregates. For example, restaurants with locations that suggest low expected mixing do not, much of the time, have low mixing: there is only a weak correlation between bridging and mixing at the level of the restaurant, despite a strong correlation at the level of the supermarket. This is because downtowns - and the bundle of amenities that define them - tend not to be situated in bridge areas but play an important role in drawing diverse groups together.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
